The XXL Survey: XLIII. The quasar radio loudness dichotomy exposed via radio luminosity functions obtained by combining results from COSMOS and XXL-S X-ray selected quasars

We studied a sample of 274 radio and X-ray selected quasars (XQSOs) detected in the COSMOS and XXL-S radio surveys at 3 GHz and 2.1 GHz, respectively. This sample was identified by adopting a conservative threshold in X-ray luminosity, Lx [2-10\ keV] >= 10^44 erg/s, selecting only the most powerful quasars. Using available multiwavelength data, we examined various criteria for the selection of radio-loud (RL) and radio-quiet (RQ) XQSOs, finding that the number of RL/RQ XQSOs changes significantly depending on the chosen criterion. This discrepancy arises due to the different criteria tracing different physical processes and due to our sample being selected from flux-limited radio and X-ray surveys. Another approach to study the origin of radio emission in XQSOs is via their radio luminosity function (RLF). We constructed the XQSO 1.4 GHz radio luminosity functions (RLFs) in six redshift bins at 0.5 <= z <= 3.7. The lower-1.4 GHz luminosity end shows a higher normalization than expected only from AGN contribution in all studied redshift bins. The found "bump" is mostly dominated by emission due to star-forming (SF) processes within the XQSO host galaxies. As expected, AGN-related radio emission dominates at the higher-luminosity end of RLF. The evolution of XQSO RLF was studied via combination of analytic forms from the literature to constrain the lower-luminosity "bump" and the higher-luminosity AGN part of the RLF. We defined two 1.4 GHz luminosity thresholds, L_th,SF and L_th,AGN, below and above which more than 80% of sources contributing to the RLF are dominated by SF and AGN-related activity, respectively. These thresholds evolve with redshift, most likely due to the strong evolution of SFRs of the XQSO host galaxies.

==> xqso_rl.tex <==
$\mathrm{L_{1.4\ GHz} = 10^{24}\ W\,Hz^{-1}}$ & 86 & 105 & 72 & 11 & 57.7 \\
$\mathrm{L_{1.4\ GHz} = 10^{25}\ W\,Hz^{-1}}$ & 16 & 175 & 51 & 32 & 24.5 \\
$\mathrm{q_{TOT} = 24 - 21.984(1+z)^{0.013}}$ & 59 & 132 & 57 & 26 & 42.3 \\
$\mathrm{R_B = 1}$ (unobscured) & 45 & 52 & 30 & 15 & 52.8 \\
$\mathrm{R_B = 1}$ (all) & 133 & 58 & 66 & 15 & 73.2 \\
$\mathrm{R_x = -3}$ & 12 & 179 & 35 & 48 & 17.2 \\

